CaLDiff: Camera Localization in NeRF via Pose Diffusion

With the widespread use of NeRF-based implicit 3D representation, the need for camera localization in the same representation becomes manifestly apparent. Doing so not only simplifies the localization process -- by avoiding an outside-the-NeRF-based localization -- but also has the potential to offer the benefit of enhanced localization. This paper studies the problem of localizing cameras in NeRF using a diffusion model for camera pose adjustment. More specifically, given a pre-trained NeRF model, we train a diffusion model that iteratively updates randomly initialized camera poses, conditioned upon the image to be localized. At test time, a new camera is localized in two steps: first, coarse localization using the proposed pose diffusion process, followed by local refinement steps of a pose inversion process in NeRF. In fact, the proposed camera localization by pose diffusion (CaLDiff) method also integrates the pose inversion steps within the diffusion process. Such integration offers significantly better localization, thanks to our downstream refinement-aware diffusion process. Our exhaustive experiments on challenging real-world data validate our method by providing significantly better results than the compared methods and the established baselines. Our source code will be made publicly available.

==> ieee_fullname.bst.tex <==
% This is a modification to the normal ieee.bst used by CVPR to render
% first names in the bibliography as "Firstname Lastname" rather than
% "F. Lastname".
%
% Jonathan T. Barron, 12/5/2018, jonbarron@gmail.com

% ---------------------------------------------------------------
%
% ieee.bst,v 1.0 2002/04/16
%
% by Glenn Paulley (paulley@acm.org)
%
% Modified from latex8.bst 1995/09/15 15:13:49 ienne Exp $
%
% by Paolo.Ienne@di.epfl.ch
%
%
% ---------------------------------------------------------------
%
% no guarantee is given that the format corresponds perfectly to 
% IEEE 8.5" x 11" Proceedings, but most features should be ok.
%
% ---------------------------------------------------------------
%
% `ieee' from BibTeX standard bibliography style `abbrv'
% version 0.99a for BibTeX versions 0.99a or later, LaTeX version 2.09.
% Copyright (C) 1985, all rights reserved.
% Copying of this file is authorized only if either
% (1) you make absolutely no changes to your copy, including name, or
% (2) if you do make changes, you name it something other than
% btxbst.doc, plain.bst, unsrt.bst, alpha.bst, and abbrv.bst.
% This restriction helps ensure that all standard styles are identical.
% The file btxbst.doc has the documentation for this style.

ENTRY
  { address
    author
    booktitle
    chapter
    edition
    editor
    howpublished
    institution
    journal
    key
    month
    note
    number
    organization
    pages
    publisher
    school
    series
    title
    type
    volume
    year
  }
  {}
  { label }

INTEGERS { output.state before.all mid.sentence after.sentence after.block }

FUNCTION {init.state.consts}
{ #0 'before.all :=
  #1 'mid.sentence :=
  #2 'after.sentence :=
  #3 'after.block :=
}

STRINGS { s t }

FUNCTION {output.nonnull}
{ 's :=
  output.state mid.sentence =
    { ", " * write$ }
    { output.state after.block =
 { add.period$ write$
   newline$
   "\newblock " write$
 }
 { output.state before.all =
     'write$
     { add.period$ " " * write$ }
   if$
 }
      if$
      mid.sentence 'output.state :=
    }
  if$
  s
}

FUNCTION {output}
{ duplicate$ empty$
    'pop$
    'output.nonnull
  if$
}

FUNCTION {output.check}
{ 't :=
  duplicate$ empty$
    { pop$ "empty " t * " in " * cite$ * warning$ }
    'output.nonnull
  if$
}

FUNCTION {output.bibitem}
{ newline$
  "\bibitem{" write$
  cite$ write$
  "}" write$
  newline$
  ""
  before.all 'output.state :=
}

FUNCTION {fin.entry}
{ add.period$
  write$
  newline$
}

FUNCTION {new.block}
{ output.state before.all =
    'skip$
    { after.block 'output.state := }
  if$
}

FUNCTION {new.sentence}
{ output.state after.block =
    'skip$
    { output.state before.all =
 'skip$
 { after.sentence 'output.state := }
      if$
    }
  if$
}

FUNCTION {not}
{   { #0 }
    { #1 }
  if$
}

FUNCTION {and}
{   'skip$
    { pop$ #0 }
  if$
}

FUNCTION {or}
{   { pop$ #1 }
    'skip$
  if$
}

FUNCTION {new.block.checka}
{ empty$
    'skip$
    'new.block
  if$
}

FUNCTION {new.block.checkb}
{ empty$
  swap$ empty$
  and
    'skip$
    'new.block
  if$
}

FUNCTION {new.sentence.checka}
{ empty$
    'skip$
    'new.sentence
  if$
}

FUNCTION {new.sentence.checkb}
{ empty$
  swap$ empty$
  and
    'skip$
    'new.sentence
  if$
}

FUNCTION {field.or.null}
{ duplicate$ empty$
    { pop$ "" }
    'skip$
  if$
}

FUNCTION {emphasize}
{ duplicate$ empty$
    { pop$ "" }
    { "{\em " swap$ * "}" * }
  if$
}

INTEGERS { nameptr namesleft numnames }

FUNCTION {format.names}
{ 's :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    % Formerly { s nameptr "{f.~}{vv~}{ll}{, jj}" format.name$ 't :=
    { s nameptr "{ff }{vv }{ll}{, jj}" format.name$ 't :=
      nameptr #1 >
 { namesleft #1 >
     { ", " * t * }
     { numnames #2 >
  { "," * }
  'skip$
       if$
       t "others" =
  { " et~al." * }
  { " and " * t * }
       if$
     }
   if$
 }
 't
      if$
      nameptr #1 + 'nameptr :=

      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {format.authors}
{ author empty$
    { "" }
    { author format.names }
  if$
}

FUNCTION {format.editors}
{ editor empty$
    { "" }
    { editor format.names
      editor num.names$ #1 >
 { ", editors" * }
 { ", editor" * }
      if$
    }
  if$
}

FUNCTION {format.title}
{ title empty$
    { "" }
    { title "t" change.case$ }
  if$
}

FUNCTION {n.dashify}
{ 't :=
  ""
    { t empty$ not }
    { t #1 #1 substring$ "-" =
 { t #1 #2 substring$ "--" = not
     { "--" *
       t #2 global.max$ substring$ 't :=
     }
     {   { t #1 #1 substring$ "-" = }
  { "-" *
    t #2 global.max$ substring$ 't :=
  }
       while$
     }
   if$
 }
 { t #1 #1 substring$ *
   t #2 global.max$ substring$ 't :=
 }
      if$
    }
  while$
}

FUNCTION {format.date}
{ year empty$
    { month empty$
 { "" }
 { "there's a month but no year in " cite$ * warning$
   month
 }
      if$
    }
    { month empty$
 'year
 { month " " * year * }
      if$
    }
  if$
}

FUNCTION {format.btitle}
{ title emphasize
}

FUNCTION {tie.or.space.connect}
{ duplicate$ text.length$ #3 <
    { "~" }
    { " " }
  if$
  swap$ * *
}

FUNCTION {either.or.check}
{ empty$
    'pop$
    { "can't use both " swap$ * " fields in " * cite$ * warning$ }
  if$
}

FUNCTION {format.bvolume}
{ volume empty$
    { "" }
    { "volume" volume tie.or.space.connect
      series empty$
 'skip$
 { " of " * series emphasize * }
      if$
      "volume and number" number either.or.check
    }
  if$
}

FUNCTION {format.number.series}
{ volume empty$
    { number empty$
 { series field.or.null }
 { output.state mid.sentence =
     { "number" }
     { "Number" }
   if$
   number tie.or.space.connect
   series empty$
     { "there's a number but no series in " cite$ * warning$ }
     { " in " * series * }
   if$
 }
      if$
    }
    { "" }
  if$
}

FUNCTION {format.edition}
{ edition empty$
    { "" }
    { output.state mid.sentence =
 { edition "l" change.case$ " edition" * }
 { edition "t" change.case$ " edition" * }
      if$
    }
  if$
}

INTEGERS { multiresult }

FUNCTION {multi.page.check}
{ 't :=
  #0 'multiresult :=
    { multiresult not
      t empty$ not
      and
    }
    { t #1 #1 substring$
      duplicate$ "-" =
      swap$ duplicate$ "," =
      swap$ "+" =
      or or
 { #1 'multiresult := }
 { t #2 global.max$ substring$ 't := }
      if$
    }
  while$
  multiresult
}

FUNCTION {format.pages}
{ pages empty$
    { "" }
    { pages multi.page.check
 { "pages" pages n.dashify tie.or.space.connect }
 { "page" pages tie.or.space.connect }
      if$
    }
  if$
}

FUNCTION {format.vol.num.pages}
{ volume field.or.null
  number empty$
    'skip$
    { "(" number * ")" * *
      volume empty$
 { "there's a number but no volume in " cite$ * warning$ }
 'skip$
      if$
    }
  if$
  pages empty$
    'skip$
    { duplicate$ empty$
 { pop$ format.pages }
 { ":" * pages n.dashify * }
      if$
    }
  if$
}

FUNCTION {format.chapter.pages}
{ chapter empty$
    'format.pages
    { type empty$
 { "chapter" }
 { type "l" change.case$ }
      if$
      chapter tie.or.space.connect
      pages empty$
 'skip$
 { ", " * format.pages * }
      if$
    }
  if$
}

FUNCTION {format.in.ed.booktitle}
{ booktitle empty$
    { "" }
    { editor empty$
 { "In " booktitle emphasize * }
 { "In " format.editors * ", " * booktitle emphasize * }
      if$
    }
  if$
}

FUNCTION {empty.misc.check}

{ author empty$ title empty$ howpublished empty$
  month empty$ year empty$ note empty$
  and and and and and
  key empty$ not and
    { "all relevant fields are empty in " cite$ * warning$ }
    'skip$
  if$
}

FUNCTION {format.thesis.type}
{ type empty$
    'skip$
    { pop$
      type "t" change.case$
    }
  if$
}

FUNCTION {format.tr.number}
{ type empty$
    { "Technical Report" }
    'type
  if$
  number empty$
    { "t" change.case$ }
    { number tie.or.space.connect }
  if$
}

FUNCTION {format.article.crossref}
{ key empty$
    { journal empty$
 { "need key or journal for " cite$ * " to crossref " * crossref *
   warning$
   ""
 }
 { "In {\em " journal * "\/}" * }
      if$
    }
    { "In " key * }
  if$
  " \cite{" * crossref * "}" *
}

FUNCTION {format.crossref.editor}
{ editor #1 "{vv~}{ll}" format.name$
  editor num.names$ duplicate$
  #2 >
    { pop$ " et~al." * }
    { #2 <
 'skip$
 { editor #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
     { " et~al." * }
     { " and " * editor #2 "{vv~}{ll}" format.name$ * }
   if$
 }
      if$
    }
  if$
}

FUNCTION {format.book.crossref}
{ volume empty$
    { "empty volume in " cite$ * "'s crossref of " * crossref * warning$
      "In "
    }
    { "Volume" volume tie.or.space.connect
      " of " *
    }
  if$
  editor empty$
  editor field.or.null author field.or.null =
  or
    { key empty$
 { series empty$
     { "need editor, key, or series for " cite$ * " to crossref " *
       crossref * warning$
       "" *
     }
     { "{\em " * series * "\/}" * }
   if$
 }
 { key * }
      if$
    }
    { format.crossref.editor * }
  if$
  " \cite{" * crossref * "}" *
}

FUNCTION {format.incoll.inproc.crossref}
{ editor empty$
  editor field.or.null author field.or.null =
  or
    { key empty$
 { booktitle empty$
     { "need editor, key, or booktitle for " cite$ * " to crossref " *
       crossref * warning$
       ""
     }
     { "In {\em " booktitle * "\/}" * }
   if$
 }
 { "In " key * }
      if$
    }
    { "In " format.crossref.editor * }
  if$
  " \cite{" * crossref * "}" *
}

FUNCTION {article}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.title "title" output.check
  new.block
  crossref missing$
    { journal emphasize "journal" output.check
      format.vol.num.pages output
      format.date "year" output.check
    }
    { format.article.crossref output.nonnull
      format.pages output
    }
  if$
  new.block
  note output
  fin.entry
}

FUNCTION {book}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check }
    { format.authors output.nonnull
      crossref missing$
 { "author and editor" editor either.or.check }
 'skip$
      if$
    }
  if$
  new.block
  format.btitle "title" output.check
  crossref missing$
    { format.bvolume output
      new.block
      format.number.series output
      new.sentence
      publisher "publisher" output.check
      address output
    }
    { new.block
      format.book.crossref output.nonnull
    }
  if$
  format.edition output
  format.date "year" output.check
  new.block
  note output
  fin.entry
}

FUNCTION {booklet}
{ output.bibitem
  format.authors output
  new.block
  format.title "title" output.check
  howpublished address new.block.checkb
  howpublished output
  address output
  format.date output
  new.block
  note output
  fin.entry
}

FUNCTION {inbook}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check }
    { format.authors output.nonnull

      crossref missing$
 { "author and editor" editor either.or.check }
 'skip$
      if$
    }
  if$
  new.block
  format.btitle "title" output.check
  crossref missing$
    { format.bvolume output
      format.chapter.pages "chapter and pages" output.check
      new.block
      format.number.series output
      new.sentence
      publisher "publisher" output.check
      address output
    }
    { format.chapter.pages "chapter and pages" output.check
      new.block
      format.book.crossref output.nonnull
    }
  if$
  format.edition output
  format.date "year" output.check
  new.block
  note output
  fin.entry
}

FUNCTION {incollection}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.title "title" output.check
  new.block
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      format.bvolume output
      format.number.series output
      format.chapter.pages output
      new.sentence
      publisher "publisher" output.check
      address output
      format.edition output
      format.date "year" output.check
    }
    { format.incoll.inproc.crossref output.nonnull
      format.chapter.pages output
    }
  if$
  new.block
  note output
  fin.entry
}

FUNCTION {inproceedings}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.title "title" output.check
  new.block
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      format.bvolume output
      format.number.series output
      format.pages output
      address empty$
 { organization publisher new.sentence.checkb
   organization output
   publisher output
   format.date "year" output.check
 }
 { address output.nonnull
   format.date "year" output.check
   new.sentence
   organization output
   publisher output
 }
      if$
    }
    { format.incoll.inproc.crossref output.nonnull
      format.pages output
    }
  if$
  new.block
  note output
  fin.entry
}

FUNCTION {conference} { inproceedings }

FUNCTION {manual}
{ output.bibitem
  author empty$
    { organization empty$
 'skip$
 { organization output.nonnull
   address output
 }
      if$
    }
    { format.authors output.nonnull }
  if$
  new.block
  format.btitle "title" output.check
  author empty$
    { organization empty$
 { address new.block.checka
   address output
 }
 'skip$
      if$
    }
    { organization address new.block.checkb
      organization output
      address output
    }
  if$
  format.edition output
  format.date output
  new.block
  note output
  fin.entry
}

FUNCTION {mastersthesis}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.title "title" output.check
  new.block
  "Master's thesis" format.thesis.type output.nonnull
  school "school" output.check
  address output
  format.date "year" output.check
  new.block
  note output
  fin.entry
}

FUNCTION {misc}
{ output.bibitem
  format.authors output
  title howpublished new.block.checkb
  format.title output
  howpublished new.block.checka
  howpublished output
  format.date output
  new.block
  note output
  fin.entry
  empty.misc.check
}

FUNCTION {phdthesis}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.btitle "title" output.check
  new.block
  "PhD thesis" format.thesis.type output.nonnull
  school "school" output.check
  address output
  format.date "year" output.check
  new.block
  note output
  fin.entry
}

FUNCTION {proceedings}
{ output.bibitem
  editor empty$
    { organization output }
    { format.editors output.nonnull }

  if$
  new.block
  format.btitle "title" output.check
  format.bvolume output
  format.number.series output
  address empty$
    { editor empty$
 { publisher new.sentence.checka }
 { organization publisher new.sentence.checkb
   organization output
 }
      if$
      publisher output
      format.date "year" output.check
    }
    { address output.nonnull
      format.date "year" output.check
      new.sentence
      editor empty$
 'skip$
 { organization output }
      if$
      publisher output
    }
  if$
  new.block
  note output
  fin.entry
}

FUNCTION {techreport}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.title "title" output.check
  new.block
  format.tr.number output.nonnull
  institution "institution" output.check
  address output
  format.date "year" output.check
  new.block
  note output
  fin.entry
}

FUNCTION {unpublished}
{ output.bibitem
  format.authors "author" output.check
  new.block
  format.title "title" output.check
  new.block
  note "note" output.check
  format.date output
  fin.entry
}

FUNCTION {default.type} { misc }

MACRO {jan} {"Jan."}

MACRO {feb} {"Feb."}

MACRO {mar} {"Mar."}

MACRO {apr} {"Apr."}

MACRO {may} {"May"}

MACRO {jun} {"June"}

MACRO {jul} {"July"}

MACRO {aug} {"Aug."}

MACRO {sep} {"Sept."}

MACRO {oct} {"Oct."}

MACRO {nov} {"Nov."}

MACRO {dec} {"Dec."}

MACRO {acmcs} {"ACM Comput. Surv."}

MACRO {acta} {"Acta Inf."}

MACRO {cacm} {"Commun. ACM"}

MACRO {ibmjrd} {"IBM J. Res. Dev."}

MACRO {ibmsj} {"IBM Syst.~J."}

MACRO {ieeese} {"IEEE Trans. Softw. Eng."}

MACRO {ieeetc} {"IEEE Trans. Comput."}

MACRO {ieeetcad}
 {"IEEE Trans. Comput.-Aided Design Integrated Circuits"}

MACRO {ipl} {"Inf. Process. Lett."}

MACRO {jacm} {"J.~ACM"}

MACRO {jcss} {"J.~Comput. Syst. Sci."}

MACRO {scp} {"Sci. Comput. Programming"}

MACRO {sicomp} {"SIAM J. Comput."}

MACRO {tocs} {"ACM Trans. Comput. Syst."}

MACRO {tods} {"ACM Trans. Database Syst."}

MACRO {tog} {"ACM Trans. Gr."}

MACRO {toms} {"ACM Trans. Math. Softw."}

MACRO {toois} {"ACM Trans. Office Inf. Syst."}

MACRO {toplas} {"ACM Trans. Prog. Lang. Syst."}

MACRO {tcs} {"Theoretical Comput. Sci."}

READ

FUNCTION {sortify}
{ purify$
  "l" change.case$
}

INTEGERS { len }

FUNCTION {chop.word}
{ 's :=
  'len :=
  s #1 len substring$ =
    { s len #1 + global.max$ substring$ }
    's
  if$
}

FUNCTION {sort.format.names}
{ 's :=
  #1 'nameptr :=
  ""
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { nameptr #1 >
 { "   " * }
 'skip$
      if$
      s nameptr "{vv{ } }{ll{ }}{  f{ }}{  jj{ }}" format.name$ 't :=
      nameptr numnames = t "others" = and
 { "et al" * }
 { t sortify * }
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {sort.format.title}
{ 't :=
  "A " #2
    "An " #3
      "The " #4 t chop.word
    chop.word
  chop.word
  sortify
  #1 global.max$ substring$
}

FUNCTION {author.sort}
{ author empty$
    { key empty$
 { "to sort, need author or key in " cite$ * warning$
   ""
 }
 { key sortify }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION {author.editor.sort}
{ author empty$
    { editor empty$
 { key empty$
     { "to sort, need author, editor, or key in " cite$ * warning$
       ""
     }
     { key sortify }
   if$
 }
 { editor sort.format.names }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION {author.organization.sort}
{ author empty$

    { organization empty$
 { key empty$
     { "to sort, need author, organization, or key in " cite$ * warning$
       ""
     }
     { key sortify }
   if$
 }
 { "The " #4 organization chop.word sortify }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION {editor.organization.sort}
{ editor empty$
    { organization empty$
 { key empty$
     { "to sort, need editor, organization, or key in " cite$ * warning$
       ""
     }
     { key sortify }
   if$
 }
 { "The " #4 organization chop.word sortify }
      if$
    }
    { editor sort.format.names }
  if$
}

FUNCTION {presort}
{ type$ "book" =
  type$ "inbook" =
  or
    'author.editor.sort
    { type$ "proceedings" =
 'editor.organization.sort
 { type$ "manual" =
     'author.organization.sort
     'author.sort
   if$
 }
      if$
    }
  if$
  "    "
  *
  year field.or.null sortify
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
}

ITERATE {presort}

SORT

STRINGS { longest.label }

INTEGERS { number.label longest.label.width }

FUNCTION {initialize.longest.label}
{ "" 'longest.label :=
  #1 'number.label :=
  #0 'longest.label.width :=
}

FUNCTION {longest.label.pass}
{ number.label int.to.str$ 'label :=
  number.label #1 + 'number.label :=
  label width$ longest.label.width >
    { label 'longest.label :=
      label width$ 'longest.label.width :=
    }
    'skip$
  if$
}

EXECUTE {initialize.longest.label}

ITERATE {longest.label.pass}

FUNCTION {begin.bib}
{ preamble$ empty$
    'skip$
    { preamble$ write$ newline$ }
  if$
  "\begin{thebibliography}{"  longest.label  * "}" *
  "\itemsep=-1pt" * % Compact the entries a little.
  write$ newline$
}

EXECUTE {begin.bib}

EXECUTE {init.state.consts}

ITERATE {call.type$}

FUNCTION {end.bib}
{ newline$
  "\end{thebibliography}" write$ newline$
}

EXECUTE {end.bib}

% end of file ieee.bst
% ---------------------------------------------------------------





==> table/chess.tex <==
\begin{tabular}{ccc}

% GT image & CaLDiff Render & Error Map \\

\multicolumn{3}{c}{\textbf{chess}} \\


\vspace{-0.3em}
\includegraphics[width=\iw]{supp-images/chess/seq-03-frame-000000.color.png--gt.png} & 
\includegraphics[width=\iw]{supp-images/chess/seq-03-frame-000000.color.png-render.png} & 
\includegraphics[width=\iw]{supp-images/chess/seq-03-frame-000000.color.png--diff.png} \\

\vspace{0.5em}
& (0.0081, 0.51) & \\

\vspace{-0.3em}
\includegraphics[width=\iw]{supp-images/chess/seq-03-frame-000243.color.png--gt.png} & 
\includegraphics[width=\iw]{supp-images/chess/seq-03-frame-000243.color.png-render.png} & 
\includegraphics[width=\iw]{supp-images/chess/seq-03-frame-000243.color.png--diff.png} \\

\vspace{0.5em}
& (0.0270, 2.78) & \\

\vspace{-0.3em}
\includegraphics[width=\iw]{supp-images/chess/seq-05-frame-000377.color.png--gt.png} & 
\includegraphics[width=\iw]{supp-images/chess/seq-05-frame-000377.color.png-render.png} & 
\includegraphics[width=\iw]{supp-images/chess/seq-05-frame-000377.color.png--diff.png} \\

\vspace{0.5em}
& (0.0605, 5.52) & \\

\vspace{-0.3em}
\includegraphics[width=\iw]{supp-images/chess/seq-03-frame-000972.color.png--gt.png} & 
\includegraphics[width=\iw]{supp-images/chess/seq-03-frame-000972.color.png-render.png} & 
\includegraphics[width=\iw]{supp-images/chess/seq-03-frame-000972.color.png--diff.png} \\

\vspace{0.5em}
& (0.2058, 37.11) & \\

% \hline \\
% \vspace{1em}
% \includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000000.color.png--gt.png} & 
% \includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000000.color.png-render.png} & 
% \includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000000.color.png--diff.png} \\


\end{tabular}

==> table/fire.tex <==
\begin{tabular}{ccc}

% GT image & CaLDiff Render & Error Map \\

\multicolumn{3}{c}{\textbf{fire}} \\


\vspace{-0.3em}
\includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000000.color.png--gt.png} & 
\includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000000.color.png-render.png} & 
\includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000000.color.png--diff.png} \\

\vspace{0.5em}
& (0.0057, 1.04) & \\

\vspace{-0.3em}
\includegraphics[width=\iw]{supp-images/fire/seq-04-frame-000458.color.png--gt.png} & 
\includegraphics[width=\iw]{supp-images/fire/seq-04-frame-000458.color.png-render.png} & 
\includegraphics[width=\iw]{supp-images/fire/seq-04-frame-000458.color.png--diff.png} \\

\vspace{0.5em}
& (0.0117, 2.69) & \\

\vspace{-0.3em}
\includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000081.color.png--gt.png} & 
\includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000081.color.png-render.png} & 
\includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000081.color.png--diff.png} \\

\vspace{0.5em}
& (0.1100, 18.33) & \\

\vspace{-0.3em}
\includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000162.color.png--gt.png} & 
\includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000162.color.png-render.png} & 
\includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000162.color.png--diff.png} \\

\vspace{0.5em}
& (0.2789, 27.08) & \\

% \hline \\
% \vspace{1em}
% \includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000000.color.png--gt.png} & 
% \includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000000.color.png-render.png} & 
% \includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000000.color.png--diff.png} \\


\end{tabular}

==> table/heads.tex <==
\begin{tabular}{ccc}

% GT image & CaLDiff Render & Error Map \\

\multicolumn{3}{c}{\textbf{heads}} \\


\vspace{-0.3em}
\includegraphics[width=\iw]{supp-images/heads/seq-01-frame-000000.color.png--gt.png} & 
\includegraphics[width=\iw]{supp-images/heads/seq-01-frame-000000.color.png-render.png} & 
\includegraphics[width=\iw]{supp-images/heads/seq-01-frame-000000.color.png--diff.png} \\

\vspace{0.5em}
& (0.0023, 0.349) & \\

\vspace{-0.3em}
\includegraphics[width=\iw]{supp-images/heads/seq-01-frame-000658.color.png--gt.png} & 
\includegraphics[width=\iw]{supp-images/heads/seq-01-frame-000658.color.png-render.png} & 
\includegraphics[width=\iw]{supp-images/heads/seq-01-frame-000658.color.png--diff.png} \\

\vspace{0.5em}
& (0.0304, 2.44) & \\

\vspace{-0.3em}
\includegraphics[width=\iw]{supp-images/heads/seq-01-frame-000376.color.png--gt.png} & 
\includegraphics[width=\iw]{supp-images/heads/seq-01-frame-000376.color.png-render.png} & 
\includegraphics[width=\iw]{supp-images/heads/seq-01-frame-000376.color.png--diff.png} \\

\vspace{0.5em}
& (0.0443, 7.78) & \\

\vspace{-0.3em}
\includegraphics[width=\iw]{supp-images/heads/seq-01-frame-000094.color.png--gt.png} & 
\includegraphics[width=\iw]{supp-images/heads/seq-01-frame-000094.color.png-render.png} & 
\includegraphics[width=\iw]{supp-images/heads/seq-01-frame-000094.color.png--diff.png} \\

\vspace{0.5em}
& (0.5316, 19.38) & \\

% \hline \\
% \vspace{1em}
% \includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000000.color.png--gt.png} & 
% \includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000000.color.png-render.png} & 
% \includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000000.color.png--diff.png} \\


\end{tabular}

==> table/naamii_stairs.tex <==
\begin{tabular}{ccc}

% GT image & CaLDiff Render & Error Map \\

\multicolumn{3}{c}{\textbf{stairs1}} \\


% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/naamii_stair/0102.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/naamii_stair/0102.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/naamii_stair/0102.jpg--diff.png} \\

\vspace{0.5em}
& (0.0034, 0.51) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/naamii_stair/0181.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/naamii_stair/0181.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/naamii_stair/0181.jpg--diff.png} \\

\vspace{0.5em}
& (0.0122, 4.44) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/naamii_stair/0188.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/naamii_stair/0188.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/naamii_stair/0188.jpg--diff.png} \\

\vspace{0.5em}
& (0.0194, 7.26) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/naamii_stair/0214.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/naamii_stair/0214.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/naamii_stair/0214.jpg--diff.png} \\

\vspace{0.5em}
& (0.1098, 29.21) & \\

\end{tabular}

==> table/room10.tex <==
\begin{tabular}{ccc}

% GT image & CaLDiff Render & Error Map \\

\multicolumn{3}{c}{\textbf{room1}} \\


% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_10/0021.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_10/0021.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_10/0021.jpg--diff.png} \\

\vspace{0.5em}
& (0.0064, 0.42) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_10/0028.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_10/0028.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_10/0028.jpg--diff.png} \\

\vspace{0.5em}
& (0.0604, 4.25) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_10/0068.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_10/0068.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_10/0068.jpg--diff.png} \\

\vspace{0.5em}
& (0.2731, 8.19) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_10/0018.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_10/0018.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_10/0018.jpg--diff.png} \\

\vspace{0.5em}
& (0.1687, 93.11) & \\

\end{tabular}

==> table/room11.tex <==
\begin{tabular}{ccc}

% GT image & CaLDiff Render & Error Map \\

\multicolumn{3}{c}{\textbf{room2}} \\


% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room11/0004.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room11/0004.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room11/0004.jpg--diff.png} \\

\vspace{0.5em}
& (0.0359, 0.53) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room11/0062.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room11/0062.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room11/0062.jpg--diff.png} \\

\vspace{0.5em}
& (0.0305, 2.52) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room11/0000.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room11/0000.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room11/0000.jpg--diff.png} \\

\vspace{0.5em}
& (0.0849, 5.3) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room11/0015.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room11/0015.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room11/0015.jpg--diff.png} \\

\vspace{0.5em}
& (0.3288, 57.34) & \\

\end{tabular}

==> table/room12.tex <==
\begin{tabular}{ccc}

% GT image & CaLDiff Render & Error Map \\

\multicolumn{3}{c}{\textbf{room3}} \\


% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room12/0018.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room12/0018.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room12/0018.jpg--diff.png} \\

\vspace{0.5em}
& (0.0100, 0.80) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room12/0016.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room12/0016.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room12/0016.jpg--diff.png} \\

\vspace{0.5em}
& (0.0258, 2.04) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room12/0003.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room12/0003.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room12/0003.jpg--diff.png} \\

\vspace{0.5em}
& (0.0319, 6.98) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room12/0000.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room12/0000.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room12/0000.jpg--diff.png} \\

\vspace{0.5em}
& (0.0625, 55.83) & \\

\end{tabular}

==> table/room_13b.tex <==
\begin{tabular}{ccc}

% GT image & CaLDiff Render & Error Map \\

\multicolumn{3}{c}{\textbf{room4}} \\


% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_13b/0271.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_13b/0271.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_13b/0271.jpg--diff.png} \\

\vspace{0.5em}
& (0.0193, 1.56) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_13b/0168.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_13b/0168.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_13b/0168.jpg--diff.png} \\

\vspace{0.5em}
& (0.0254, 2.25) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_13b/0055.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_13b/0055.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_13b/0055.jpg--diff.png} \\

\vspace{0.5em}
& (0.1231, 9.97) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_13b/0163.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_13b/0163.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_13b/0163.jpg--diff.png} \\

\vspace{0.5em}
& (0.3215, 42.85) & \\

\end{tabular}

==> table/room_14a.tex <==
\begin{tabular}{ccc}

% GT image & CaLDiff Render & Error Map \\

\multicolumn{3}{c}{\textbf{room5}} \\


% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_14a/0142.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_14a/0142.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_14a/0142.jpg--diff.png} \\

\vspace{0.5em}
& (0.0025, 0.06) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_14a/0276.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_14a/0276.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_14a/0276.jpg--diff.png} \\

\vspace{0.5em}
& (0.0163, 2.88) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_14a/0159.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_14a/0159.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_14a/0159.jpg--diff.png} \\

\vspace{0.5em}
& (0.0590, 8.20) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_14a/0263.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_14a/0263.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_14a/0263.jpg--diff.png} \\

\vspace{0.5em}
& (0.2801, 41.00) & \\

\end{tabular}

==> table/room_15a.tex <==
\begin{tabular}{ccc}

% GT image & CaLDiff Render & Error Map \\

\multicolumn{3}{c}{\textbf{room6}} \\


% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_15a/0214.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_15a/0214.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_15a/0214.jpg--diff.png} \\

\vspace{0.5em}
& (0.0185, 1.83) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_15a/0102.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_15a/0102.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_15a/0102.jpg--diff.png} \\

\vspace{0.5em}
& (0.0162, 2.14) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_15a/0363.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_15a/0363.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_15a/0363.jpg--diff.png} \\

\vspace{0.5em}
& (0.1326, 14.67) & \\

% \vspace{-0.3em}
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_15a/0192.jpg--gt.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_15a/0192.jpg-render.png} & 
\includegraphics[width=\iw,angle=-90,origin=c]{supp-images/room_15a/0192.jpg--diff.png} \\

\vspace{0.5em}
& (0.1090, 99.17) & \\

\end{tabular}

==> table/stairs.tex <==
\begin{tabular}{ccc}

% GT image & CaLDiff Render & Error Map \\

\multicolumn{3}{c}{\textbf{stairs}} \\


\vspace{-0.3em}
\includegraphics[width=\iw]{supp-images/stairs/seq-01-frame-000356.color.png--gt.png} & 
\includegraphics[width=\iw]{supp-images/stairs/seq-01-frame-000356.color.png-render.jpeg} & 
\includegraphics[width=\iw]{supp-images/stairs/seq-01-frame-000356.color.png--diff.png} \\

\vspace{0.5em}
& (0.0766, 1.53) & \\

\vspace{-0.3em}
\includegraphics[width=\iw]{supp-images/stairs/seq-01-frame-000267.color.png--gt.png} & 
\includegraphics[width=\iw]{supp-images/stairs/seq-01-frame-000267.color.png-render.png} & 
\includegraphics[width=\iw]{supp-images/stairs/seq-01-frame-000267.color.png--diff.png} \\

\vspace{0.5em}
& (0.1011, 3.27) & \\

\vspace{-0.3em}
\includegraphics[width=\iw]{supp-images/stairs/seq-01-frame-000089.color.png--gt.png} & 
\includegraphics[width=\iw]{supp-images/stairs/seq-01-frame-000089.color.png-render.png} & 
\includegraphics[width=\iw]{supp-images/stairs/seq-01-frame-000089.color.png--diff.png} \\

\vspace{0.5em}
& (0.1015, 7.80) & \\

\vspace{-0.3em}
\includegraphics[width=\iw]{supp-images/stairs/seq-01-frame-000000.color.png--gt.png} & 
\includegraphics[width=\iw]{supp-images/stairs/seq-01-frame-000000.color.png-render.png} & 
\includegraphics[width=\iw]{supp-images/stairs/seq-01-frame-000000.color.png--diff.png} \\

\vspace{0.5em}
& (0.1791, 16.84) & \\

% \hline \\
% \vspace{1em}
% \includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000000.color.png--gt.png} & 
% \includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000000.color.png-render.png} & 
% \includegraphics[width=\iw]{supp-images/fire/seq-03-frame-000000.color.png--diff.png} \\


\end{tabular}

==> text/archive.tex <==
\clearpage
\section{Introduction Archive}
\textcolor{blue}{
\textbf{Comments from Danda:}
1) The teaser figure, figure 1 must be about qualitative results with poor texture.. hopefully making the reason of H-Loc to fail and our method to succeed intuitive! 2)  Figure 2 must have current have the current figure 1 with integrated iNeRF. Figure 2 will have three parts: two parts of training and one of the inference. In two parts of training, the diffusion part will be highlighted more than the iNerf part (current fig 1 vs. fig 2).
3) Please, focus on including experimental results and implementation details! 4) BTW, what happened to the other baselines that Bishad was exploring previously? 5) what happens if you train only on the rendered images?
}

Visual localization is referred to as the process of determining the position of a camera within a known scene, such as a 3D map. It is a crucial component for a wide range of applications, including autonomous vehicle navigation, mobile robotics, augmented reality, and Structure-from-Motion (SfM).

\old{The ability to estimate a camera pose from an image is a fundamental requirement for many computer vision applications, including autonomous vehicle navigation, mobile robotics, augmented reality, and structure-from-motion (SfM).} 

\FR{Notes:
\begin{itemize}
    \item Sorry, my version is way to detailed for an intro, it makes it boring haha we can keep that a bit for the literature review, maybe.
    \item Also I have another problem here is that we basically "defend" end-to-end approach while we are not end to end strictly speaking? are we?
    \item  Maybe the NeRF intro part should come before? 
    \item Also how do we justify the diffusion part?
\end{itemize}}

Localization process can operate at varying levels of granularity to provide either an approximate position of the camera or an exact 6DoF (six degrees of freedom) pose estimate. Most effective and accurate techniques employ a hierarchical strategy [], where localization is approached in two successive and complementary steps: initially, coarse localization is achieved using an image retrieval method [] to narrow the search range. This is followed by fine pose estimation, which involves a local descriptor matching [] strategy. While these approaches have demonstrated their relevance for challenging outdoor environments, their accuracy remains limited in indoor textureless environments. In contrast, end-to-end deep learning-based approaches such as PoseNet~\cite{kendall2015posenet} demonstrated better resilience under such conditions. 

\old{Hierarchical Localization based approaches are widely used to solve the problem of image-based localization. These approaches rely on local handcrafted features such as SIFT, SURF, ORB or learned features such as SuperPoint, DISK \FR{Too detailed, just mention "local keypoint extraction" and just add one reference or a survey on those techniques}. Learned features have shown significantly better results over the handcrafted method. However, feature detection and matching can get severely impacted if the environment has less texture. In contrast, end-to-end deep learning based approaches such as PoseNet~\cite{kendall2015posenet} do not care about the environment textures and directly provide an output pose for a given image. PoseNet formulates 6DoF pose estimation as a regression problem, but is significantly less accurate than Hierarchical Localization based approach.}

\FR{Here one fundamental questions, why is it important to localize a camera in a Nerf?}
The emergence of Neural Radiance Fields (NeRF) has opened up new possibilities for object pose estimation. NeRF and its variants learn generative models of objects from pose-annotated image collections, capturing complex 3D structures and high-fidelity surface details. iNeRF is an analysis-by-synthesis approach for pose estimation built on the concept of inverting a NeRF model. Inspired by iNeRF’s success, this paper further explores the idea of pose estimation via neural radiance field inversion. However, NeRF’s computational overhead can impact execution time. To overcome this limitation, we leverage our fast version of NeRF, known as Instant Neural Graphics Primitives (Instant NGP). Using Instant NGP model inversion provides significant speedups over NeRF. The structure of Instant NGP admits parallel optimization, which is leveraged to overcome issues with local minima and thereby achieve greater robustness than possible with iNeRF. Similar to iNeRF, our pose estimation requires three inputs: a single RGB image with the target, an initial rough pose estimate of the target, and an instant NGP model trained from multiple views.

Diffusion models have been shown to generate high-quality samples from complex distributions and have delivered encouraging results in audio synthesis and image applications. These models can be conditioned on anything to produce different data distributions for different conditions. We formulate the Camera Pose as Point Distribution conditioned on the Image taken from that pose. With sufficient image-pose pairs, the diffusion model can generalize to produce camera pose of unseen images. 

In summary, this work makes the following contributions:
\begin{itemize}
    \item Iterative pose refinement using diffusion models works significantly better than single step PoseNet like method.
    \item Integrating the pose inversion steps within the diffusion process helps to increase the localization accuracy.
    \item CaLDiff has significant advantage over the feature based hierarchical localization approach, specially for challenging environments like low texture.
\end{itemize}

\section{Method Archive}

\subsection{The method structure}
\subsubsection{Pose Initialization}
$\mathcal{P}_N=\{\mathbf{P}_T^i\}_{i=0}^n$
\subsubsection{Conditioning Feature }
$\psi_\rho(\mathbf{I})\rightarrow\mathbf{f}$
\subsubsection{Pose Diffusion}
$\phi_\theta(\mathbf{P}_t,\mathbf{f},t)\rightarrow \mathbf{P}_{t-1}$ which eventually gives us  $\mathcal{P}_0=\{\mathbf{P}_0^i\}$
\subsection{Subset Selection}
selects $\mathcal{P}_s\subset \mathcal{P}_0$
\subsection{Pose Refinement}
$\mathcal{P}_s \rightarrow \mathcal{P}_f\rightarrow\mathbf{P}_f$

\section{Experiments Archive}

\underline{What is our method?}\\
-- integrated iNeRF\\
-- post refinement

\begin{table}[]
\begin{tabular}{lll}
\hline
\textbf{ without post-refinement and integrated iNeRF}\\
\textbf{ without post-refinement}\\
\textbf{ final method}
\end{tabular}
\caption{Ablation study. Report the added time on one column.}
\end{table}

\subsection{Behaviour analysis}
\begin{itemize}
    \item How many particles
    \item how many images
    \item how many diffusion steps
    \item how much erros
    \item how much time
\end{itemize}
\textbf{How many vs. how much-- two plots before and after refinements..}


